Inverse Design of Multi-band Reflective Polarizing Metasurfaces Using Generative Machine Learning

Electromagnetic linear-to-circular polarization converters with wide- and multi-band capabilities can simplify antenna systems where circular polarization is required. Multi-band solutions are attractive in satellite communication systems, which commonly have the additional requirement that the sense of polarization is reversed {between adjacent bands}. However, the design of these structures using conventional \textit{ad hoc} methods relies heavily on empirical methods. Here, we employ a data-driven approach integrated with a generative adversarial network to explore the design space of the polarizer meta-atom thoroughly. Dual-band and triple-band reflective polarizers with stable performance over incident angles up to and including $30^\circ$, {corresponding to typical reflector antenna system requirements}, are synthesized using the proposed method. The feasibility and performance of the designed polarizer is validated through measurements of a fabricated prototype.

==> bios.tex <==
\begin{figure}
  \includegraphics[width=0.25\textwidth]{headshots/Parinaz Naseri-headshot.png}
  \caption*{Parinaz Naseri received the B.Sc. degree from the University of Tehran, Iran, in 2013, and the M.Sc. degree from the University of Alberta, Canada, in 2017, both in electrical and computer engineering. In 2016, she was a recipient of a research fellowship at the Instituto de Telecomunicações, Portugal, to work on European Space Agency-funded projects for metasurface-based solutions for satellite communications. In 2018, Naseri joined the Reconfigurable Antenna Laboratory, University of Toronto, as a researcher and to pursue the Ph.D. degree.  

Naseri was a recipient of the Stanley G. Jones Master’s Scholarship in 2014, Ontario Trillium Scholarship in 2018, Donald R. Studney Electromagnetics Graduate Award, IEEE AP-S Doctoral Grant in 2020, and Mojgan Daneshmand Grant in 2022. She is the organizer and, since October 2020, chair of the IEEE AP-S University of Toronto Student Branch Chapter. She also serves as a technical reviewer for several IEEE journals and conferences. }
\end{figure}

\begin{figure}
  \includegraphics{bio-placeholder.jpg}
  \caption*{Biography}
\end{figure}

\begin{figure}
  \includegraphics{bio-placeholder.jpg}
  \caption*{Biography}
\end{figure}

\begin{figure}
  \includegraphics[width=0.25\textwidth]{headshots/Sean Hum-headshot.png}
  \caption*{Sean V. Hum received the B.Sc., M.Sc., and Ph.D. degrees in electrical and computer engineering from the University of Calgary, Calgary, AB, Canada, in 1999, 2001, and 2006, respectively.

In 2006, he joined The Edward S. Rogers Senior Department of Electrical and Computer Engineering, University of Toronto (UofT), Toronto, ON, Canada, where he is currently a Professor and the Eugene V. Polistuk Chair in Electromagnetic Design. He was the Associate Chair, Graduate Studies in the same department, from 2018-2021. He leads the Reconfigurable Antenna Laboratory, UofT, and along with his students, conducts research in the areas of advanced electromagnetic surfaces, reconfigurable/multifunction antennas, space-fed arrays, and antennas for space applications.

Dr. Hum was a recipient of the Governor General’s Gold Medal for his work on radio-on-fiber systems in 2001, the IEEE Antennas and Propagation Society Student Paper Award for his work on electronically tunable reflectarrays in 2004, the ASTech Leaders of Tomorrow Award for his work in this area in 2006, the Early Researcher Award from the Government of Ontario in 2012. On the teaching side, he has been the recipient of departmental teaching awards and a Faculty Early Career Teaching Award. He was a co-recipient of the IEEE Antennas and Propagation Society R. W. P. King Award in 2015 and 2017. He served on the Steering Committee and the Technical Program Committee of the 2010 and 2020 IEEE AP-S International Symposium on Antennas and Propagation. He was the TPC Co-Chair of the 2015 IEEE AP-S International Symposium on Antennas and Propagation. He served as an Associate Editor for the IEEE Transactions on Antennas and Propagation from 2010 to 2017. He is currently co-chair of the IEEE AP-S Education Committee.}
\end{figure}

\begin{figure}
\textbf{Table of Contents}\\
\medskip
  \includegraphics{toc-image.png}
  \medskip
  \caption*{ToC Entry}
\end{figure}


==> sections/Acknowledgements.tex <==
\section*{Acknowledgements (not compulsory)}

Acknowledgements should be brief, and should not include thanks to anonymous referees and editors, or effusive comments. Grant or contribution numbers may be acknowledged.

==> sections/Additional.tex <==
\section*{Additional information}

To include, in this order: \textbf{Accession codes} (where applicable); \textbf{Competing interests} (mandatory statement). 

The corresponding author is responsible for submitting a \href{http://www.nature.com/srep/policies/index.html#competing}{competing interests statement} on behalf of all authors of the paper. This statement must be included in the submitted article file.

==> sections/Authors.tex <==
\section*{Author contributions statement}

Must include all authors, identified by initials, for example:
A.A. conceived the experiment(s),  A.A. and B.A. conducted the experiment(s), C.A. and D.A. analysed the results.  All authors reviewed the manuscript. 

==> sections/Methods.tex <==
\section*{Methods}

%\subsection*{Simulation of the unit cell.} Full-wave electromagnetic simulations are performed using the Ansoft High Frequency Structure Simulator (HFSS) commercial software. A single unit cell is simulated in a three dimensional environment by assigning Floquet ports on its top and bottom surfaces for normal and oblique incident plane-wave excitation and terminating its sides by periodic boundary conditions to simulate an infinite array. 

%\subsection*{Machine learning model developments.} 

%The implementation and training of the machine learning models are done using TensorFlow-backend Keras libraries in Python. To train the GAN, the gradients of the loss function in \Cref{eq:binaryCrossEnt} are \textit{back-propagated} to the generator and discriminator to update the weights of both networks.  

\subsection*{TRL Calibration of the quasi-optical measurement setup.} To characterize the device under test (DUT), i.e. the polarizer, under normal incidence using the quasi-optical setup, a standard four-port thru-reflect-line (TRL) calibrations is performed. Three transmission modes between the vertical (V) and horizontal (H) ports of the Tx and Rx sides of the setup are defined: V to V, H to H, and V to H. For each of these cases, three standards as thru, reflection, and line are measured. Thru standard is measured when there is nothing in between the Tx and Rx sides. Reflection standard is measured when there is a copper plate in the middle of the Tx and Rx sides. Finally, the line standard is measured when the horn and the lens on either the Rx or Tx side are moved together for a free-space quarter-wavelength when there is nothing n between the Tx and Rx sides. The horn antennas, lenses, and the DUT are all placed on micrometer translation stages for accurate movements. It is worth noting that for the V to H transmission mode, one of the horns has to be rotated by $90^\circ$ for all the three standard measurements, otherwise the signal would be in noise level. Once the calibration is completed, the plane in the middle of the Rx and Tx side is indicated as the reference plane and that is where the DUT should be placed. Furthermore, to filter out the unwanted reflections from the lenses and horn antennas, time gating has been applied for all S-parameter measurements. We note that care must be taken when positioning the metal plate to define the reflect standard for Tx and Rx antennas especially at high frequencies. Similarly, one must ensure using a consistent line standard (the free-space quarter-wavelength line) for all ports. This is because any slight deviation translates to large artificial refection and transmission phases which have strong influence on the measured values, especially on the axial ratio measurements. For the case that the horns are single-linearly polarized, a two-port TRL calibration is performed where only one transmission mode is defined and the three thru, reflection, and line standards are measured only once. 



